Improved Stabilizer Estimation via Bell Difference Sampling

We study the complexity of learning quantum states in various models with respect to the stabilizer formalism and obtain the following results: - We prove that $\Omega(n)$ $T$-gates are necessary for any Clifford+$T$ circuit to prepare computationally pseudorandom quantum states, an exponential improvement over the previously known bound. This bound is asymptotically tight if linear-time quantum-secure pseudorandom functions exist. - Given an $n$-qubit pure quantum state $|\psi\rangle$ that has fidelity at least $\tau$ with some stabilizer state, we give an algorithm that outputs a succinct description of a stabilizer state that witnesses fidelity at least $\tau - \varepsilon$. The algorithm uses $O(n/(\varepsilon^2\tau^4))$ samples and $\exp\left(O(n/\tau^4)\right) / \varepsilon^2$ time. In the regime of $\tau$ constant, this algorithm estimates stabilizer fidelity substantially faster than the na\"ive $\exp(O(n^2))$-time brute-force algorithm over all stabilizer states. - In the special case of $\tau > \cos^2(\pi/8)$, we show that a modification of the above algorithm runs in polynomial time. - We exhibit a tolerant property testing algorithm for stabilizer states. The underlying algorithmic primitive in all of our results is Bell difference sampling. To prove our results, we establish and/or strengthen connections between Bell difference sampling, symplectic Fourier analysis, and graph theory.

==> macros.tex <==
\usepackage{amsmath, amsthm, amssymb, amsfonts, braket, complexity, enumerate, mathrsfs, tikz, caption, subcaption, xcolor, mathtools, braket, dirtytalk}

\usepackage{tabularx}

\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\SetKwInput{KwInput}{Input}                %
\SetKwInput{KwOutput}{Output}
\SetKwFor{RepTimes}{repeat}{times}{end}

\usepackage[pagebackref,colorlinks,citecolor=blue,linkcolor=magenta,bookmarks=true]{hyperref}
\usepackage[nameinlink,capitalize]{cleveref}


\newcommand{\nn}{\nonumber\\}
\newcommand{\lam}{\lambda}
\newcommand{\dleta}{\delta}
\newcommand{\vphi}{\varphi}
\newcommand{\bdry}{\partial}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\lv}{\lvert}
\newcommand{\rv}{\rvert}
\newcommand{\lV}{\lVert}
\newcommand{\rV}{\rVert}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ot}{\otimes}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\zo}{\{0,1\}}
\newcommand{\F}{\mathbb{F}}
\renewcommand{\hat}{\widehat}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\bits}{\{-1,1\}}
\newcommand{\tf}{\{\true, \false\}}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{question}[theorem]{Question}
\newcommand{\stab}{\textrm{Stab}}
\newcommand{\stabset}{\mathcal{S}}
\newcommand{\stabbasis}{\mathcal{B}}
\newcommand{\stabilizer}[1]{\ket{\varphi_{#1}}}
\newcommand{\bstabilizer}[1]{\bra{\varphi_{#1}}}
\newcommand{\pmone}{\{\pm 1\}}
\newcommand{\intpmone}{[-1,1]}
\newcommand{\bool}{\{0, 1\}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\mc}{\mathcal}
\newcommand{\eps}{\varepsilon}
\newcommand{\labs}{\left|}
\newcommand{\rabs}{\right|}
\newcommand{\lpar}{\left(}
\newcommand{\rpar}{\right)}
\newcommand{\lbrak}{\left[}
\newcommand{\rbrak}{\right]}
\newcommand{\trnc}{\func{trnc}}
\newcommand{\sgn}{\func{sgn}}
\newcommand{\stabrank}{\chi}
\newcommand{\extent}{\xi}
\newcommand{\fidelity}{F}
\newcommand{\perm}{\func{Perm}}
\newcommand{\T}{\intercal}
\newcommand{\adj}{\dagger}

\newcommand{\had}{\textrm{H}}
\newcommand{\tgate}{\textrm{T}}
\newcommand{\cnot}{\textrm{CNOT}}
\newcommand{\pgate}{\textrm{P}}
\newcommand{\rgate}{\textrm{R}}
\newcommand{\xgate}{\textrm{X}}
\newcommand{\ygate}{\textrm{Y}}
\newcommand{\zgate}{\textrm{Z}}

\newcommand{\property}{\mathcal{P}}
\newcommand{\dist}{\func{dist}}

\renewcommand{\Pr}{\mathop{\bf Pr\/}}
\newcommand{\Ex}{\mathop{\bf E\/}}
\newcommand{\Es}[1]{\mathop{\bf E\/}_{{\substack{#1}}}}            %
\newcommand{\Var}{\mathop{\bf Var\/}}
\newcommand{\Cov}{\mathop{\bf Cov\/}}
\newcommand{\stddev}{\mathop{\bf stddev\/}}
\newcommand{\littlesum}{\mathop{{\textstyle \sum}}}
\newcommand{\littleprod}{\mathop{{\textstyle \prod}}}
\newcommand{\apx}{\mathop{\approx}}
\let\oldRe\Re
\renewcommand\Re{\mathop{\mathrm{Re}}}
\newcommand{\tr}{\mathrm{tr}} \newcommand{\Tr}{\tr} \newcommand{\trace}{\tr}
\newcommand{\size}{\mathrm{size}}
\newcommand{\avg}{\mathop{\mathrm{avg}}}
\newcommand{\odd}{\mathrm{odd}}
\newcommand{\even}{\mathrm{even}}
\newcommand{\hamdist}{\mathrm{Dist}}
\newcommand{\step}{\mathrm{step}}
\newcommand{\spn}{\mathrm{span}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\Aut}{\mathrm{Aut}}
\newcommand{\codim}{\operatorname{codim}}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\Abs}[1]{\Bigl\lvert #1 \Bigr\rvert}
\newcommand{\ABS}[1]{\left\lvert #1 \right\rvert}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\Norm}[1]{\Bigl\lVert #1 \Bigr\rVert}
\newcommand{\NORM}[1]{\left\lVert #1 \right\rVert}
\newcommand{\paren}[1]{( #1 )}
\newcommand{\Paren}[1]{\Bigl( #1 \Bigr)}
\newcommand{\PAREN}[1]{\left( #1 \right)}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ketbra}[2]{\ket{#1}\!\!\bra{#2}}

\newcommand{\sampcomplexity}[1]{O({#1}^{12})}
